D4: Detection of Adversarial Diffusion Deepfakes Using Disjoint Ensembles

Detecting diffusion-generated deepfake images remains an open problem. Current detection methods fail against an adversary who adds imperceptible adversarial perturbations to the deepfake to evade detection. In this work, we propose Disjoint Diffusion Deepfake Detection (D4), a deepfake detector designed to improve black-box adversarial robustness beyond de facto solutions such as adversarial training. D4 uses an ensemble of models over disjoint subsets of the frequency spectrum to significantly improve adversarial robustness. Our key insight is to leverage a redundancy in the frequency domain and apply a saliency partitioning technique to disjointly distribute frequency components across multiple models. We formally prove that these disjoint ensembles lead to a reduction in the dimensionality of the input subspace where adversarial deepfakes lie, thereby making adversarial deepfakes harder to find for black-box attacks. We then empirically validate the D4 method against several black-box attacks and find that D4 significantly outperforms existing state-of-the-art defenses applied to diffusion-generated deepfake detection. We also demonstrate that D4 provides robustness against adversarial deepfakes from unseen data distributions as well as unseen generative techniques.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sec/2_related.tex <==
\section{Background and Related Work}\label{sec:related_work}
\noindent\textbf{Notation.} We consider a distribution $\mathcal{D}$ over $\mathcal{X} \times \mathcal{Y}$, where $\mathcal{X} \subseteq \mathbb{R}^d$ is the input space and $\mathcal{Y} \subseteq \mathbb{Z}^c$ is the finite class-label space. We denote vectors in boldface (e.g., $\mathbf{x}$). We denote a trained classifier as a function $\mathcal{F}: \mathcal{X} \rightarrow\mathcal{Y}$ (the classifier is usually parameterized by its weights $w$, omitted for brevity). We denote the loss function as $\mathcal{L}(\mathbf{x},y)$. An ensemble classifier is a function $M_{(\mathcal{F}_1,\mathcal{F}_2,...,\mathcal{F}_n)}: \mathcal{X} \rightarrow \mathcal{Y}$ that combines the logit outputs $l_1,l_2,...,l_n$ of multiple classifiers $\mathcal{F}_1,\mathcal{F}_2,...,\mathcal{F}_n$ with a voting aggregation function $\mathcal{A}: \mathbb{R}^{n \times c} \rightarrow \mathcal{Y}$. 
% For binary classification (deepfake vs. clean), we consider two voting mechanisms: (1) majority, where the ensemble outputs the class predicted by majority of classifiers, and (2) at-least-one, where the classifier outputs deepfake label if at least one classifier predicts deepfake (else it outputs clean).

We now provide a definition for adversarial examples against a classifier. For a classifier $\mathcal{F}$ and input-label pair $(\mathbf{x},y)$, an adversarial example is a perturbed input $\mathbf{x'}$ such that (1) $\mathbf{x'}$ is misclassified, i.e., $\mathcal{F}(\mathbf{x'}) \neq y$ and (2) $||\mathbf{x} - \mathbf{x'}||$ is within a small $\epsilon$ ball, where $||.||$ is a given norm. The value of $\epsilon$ is chosen to be small so that the perturbation is imperceptible to humans.  

%Let classification model $\mathcal{F}$ (typically implemented via a neural network) be a function that performs the mapping $\mathcal{F}: \mathcal{X} \rightarrow \mathcal{Y}$. Specifically, given input $\mathbf{x} \in \mathcal{X}$ (vectors are denoted in boldface), model $\mathcal{F}$ computes the final label as the maximum a posteriori estimate from distribution $P(y \in \mathcal{Y}~|~\mathbf{x} \in \mathcal{X})$. This distribution is learnt via minimizing a loss function $\mathcal{L}_{\mathcal{F}}$ with respect to model parameters $\mathcal{W}$.
% In the {\it empirical risk
%   minimization (ERM)} framework we wish to solve the following
% optimization problem:
% \[
% \min_{w \in \mathcal{H}} \; E_{(\mathbf{x},y) \sim \mathcal{D}} \; \mathcal{L}(w,\mathbf{x},y)
% \]
% In the equation given above $\mathcal{H}$ is the hypothesis space and $\mathcal{L}$ is
% the loss function.  Since the distribution is usually unknown, a learner solves
% the following problem over a data set $S=\{ (\mathbf{x_1},y_1),
% \cdots. (\mathbf{x_n},y_n) \}$ sampled from the distribution $\mathcal{D}$.
% \[
% \min_{ w \in \mathcal{H} } \; \frac{1}{n} \sum_{i=1}^n  \mathcal{L}(w,\mathbf{x_i},y_i)
% \]
% Once we have solved the optimization problem given above, we obtain a
% $w^* \in \mathcal{H} $ which yields a classifier 

%\subsection{GANs and Deepfakes}
%Deepfakes broadly refer to digital media generated/modified by a DNN. In this work, we focus on deepfake images generated by the GAN family of DNNs. A GAN comprises a pair of networks --- a generator $\mathcal{G}$ and discriminator $\mathcal{D}$. These networks are trained in tandem with one another, i.e., $\mathcal{G}$ learns to generate realistic images from input space $\mathcal{X}$, and the $\mathcal{D}$ learns to provide $\mathcal{G}$ with feedback regarding the quality of generated images, so that it may improve. Recent work has significantly advanced the state-of-the-art for GANs~\cite{karras2019style,karras2018progressive,brock2018large,park2019semantic,zhu2017unpaired,choi2018stargan}, thereby enabling the generation of hyper-realistic deepfake images.

% A generative model is a function $G: \mathcal{Z}
%  \rightarrow \cal\mathcal{X}$, where $\mathcal{Z}$ and $\mathcal{X}$ are the latent and input spaces respectively. Such a model implicitly defines a probability distribution over the samples $G(\mathbf{z})$ for $\mathbf{z} \sim \mathcal{Z}$. Thus, we can sample over $\mathcal{Z}$ to generate samples in the input space $\mathcal{X}$.
 
% Such generators were initially difficult to train until Goodfellow et al.~\cite{goodfellow2014generative} first introduced the notion of a Generative Adversarial Network (GAN) as a way of training such generators in an adversarial network framework. Specifically, they posed the problem as a min-max game between a generator attempting to recreate a given data distribution and a discriminator attempting to differentiate inputs from the generator versus from the true distribution. Such networks have since been adapted to create fake images, known as deepfakes~\cite{karras2018progressive,karras2019style,brock2018large,park2019semantic,zhu2017unpaired,choi2018stargan}. We are interested in robust detection of images generated from such GANs.
% A generative model is a function $G: \mathcal{Z}
%  \rightarrow \cal\mathcal{X}$, where $\mathcal{Z}$ and $\mathcal{X}$ are the latent and input spaces respectively. Such a model implicitly defines a probability distribution over the samples $G(\mathbf{z})$ for $\mathbf{z} \sim \mathcal{Z}$. Thus, we can sample over $\mathcal{Z}$ to generate samples in the input space $\mathcal{X}$.
 
% Such generators were initially difficult to train until Goodfellow et al.~\cite{goodfellow2014generative} first introduced the notion of a Generative Adversarial Network (GAN) as a way of training such generators in an adversarial network framework. Specifically, they posed the problem as a min-max game between a generator attempting to recreate a given data distribution and a discriminator attempting to differentiate inputs from the generator versus from the true distribution. Such networks have since been adapted to create fake images, known as deepfakes~\cite{karras2018progressive,karras2019style,brock2018large,park2019semantic,zhu2017unpaired,choi2018stargan}. We are interested in robust detection of images generated from such GANs.


\noindent\textbf{Deepfake Image Detection.}
\nm{Need to rework this para to talk about diffusion deepfakes and not GAN deepfakes. But the flow is the same.} The research community has made rapid progress towards detecting GAN-generated deepfake images. Examples of proposed detection schemes include DNN classifiers~\citep{wang2020cnn,yu2019attributing}, color-space anomaly detection~\citep{mccloskey2018detecting}, and co-occurrence matrix analysis~\citep{nataraj2019detecting}, amongst others~\citep{tariq2019gan, mi2020gan, marra2018detection, guarnera2020deepfake, marra2019incremental}. 

A recent line of work has significantly advanced the state-of-the-art for deepfake detection by leveraging \textit{frequency-space analysis}. For example,~\citet{frank2020leveraging} proposed the idea of detecting deepfakes with the Discrete Cosine Transform (DCT) as a pre-processing transform before a binary DNN-based deepfake classifier. Similar work has also achieved remarkable performance --- ~\citet{zhang2019detecting} use GAN simulators to extract similar frequency artifacts, and~\citet{durall2019unmasking} successfully train DNNs in the frequency domain to detect deepfakes. 

\noindent\textbf{Adversarial Deepfakes.} Unfortunately, the aforementioned detectors have been rendered ineffective in adversarial settings. Specifically, ~\citet{carlini2020evading} showed that  frequency-based detectors are vulnerable to adversarial examples --- an adversary can add imperceptible adversarial perturbations to a deepfake that evade such detectors, rendering them ineffective. Others have corroborated this observation~\citep{hussain2021adversarial, hussain2022exposing, neekhara2021adversarial, gandhi2020adversarial, vo2022adversarial, shahriyar2022evaluating, fernandes2020adversarial, liao2021imperceptible, hussain2022reface}.

An adversary can construct these adversarial deepfakes in either a white-box setting (with complete knowledge of the detector's weights and parameters), or black-box setting (with only query access to the detector). In this work, we focus on robust detection in the black-box setting. The motivation for this focus is twofold. \textit{First}, deepfake detectors in the real world are likely to be black-box services, such as those already offered by Intel~\cite{}, Deepware~\cite{}, Reality Defender~\cite{} and Sensity AI~\cite{}. These services are typically available through web-based platforms or through API access. \textit{Second}, defending against white-box attacks is an extremely challenging open problem on even non-deepfake tasks, and we find that existing robust deepfake detectors are completely broken under this setting, e.g.., succumb to a 100\% attack success rate under the white-box AutoAttack benchmark (see Appendix~\ref{} for details). We thus leave defense in the white-box setting to future work.


%Subsequently, there have been initial attempts at defending against adversarial deepfakes. Inference-time defenses focus on removing the effect of the adversarial perturbation without any changes made to the detection technique --- unfortunately, these approaches are computationally intensive, e.g., upto 30 minutes per image~\citep{gandhi2020adversarial, jiang2021residual}.
%Initial attempts at defending against adversarial deepfakes have proposed inference-time defenses --- unfortunately, these approaches are computationally intensive, e.g., upto 30 minutes per image~\citep{gandhi2020adversarial, jiang2021residual}.
%Another class of defenses have considered traditional ensembles (of multiple DNNs)~\citep{dutta2021ensembledet} --- our discussion towards the end of this section highlights the shortcomings of such standard ensembling, i.e., sharing of non-robust features.    % Our work targets this limitation by improving the adversarial robustness of deepfake detection (see Section~\ref{sec:motivation_design} for detailed methodology). % We propose \name, a framework that leverages the DCT-induced frequency spectrum by intelligently distributing frequency components amongst multiple models to create an ensemble of performant detectors.

% In contrast to existing frequency based defenses, we create split subpaces within the DCT space to create ensembles that are more robust to adversarial examples. Specifically, we leverage disjoint DCT regions to train an ensemble of models with orthogonal gradients. 

%\subsection{Adversarial Examples}


% DNN based models have been shown to be vulnerable to these slightly perturbed adversarial examples, first shown on image classification models~\cite{biggio2013evasion,goodfellow2015explaining,szegedy2014intriguing}. Common techniques include the PGD-$k$ attack~\cite{madry2018towards}, where $k$ denotes the number of steps, and the Carlini-Wagner attack~\cite{carlini2017towards}. Such techniques discover perturbations be taking small steps in a gradient direction to increase the classification error.

%As such, many DNN-based image classifiers have been shown to be vulnerable to adversarial examples~\cite{szegedy2014intriguing,goodfellow2015explaining,biggio2013evasion}. In fact, recent work from Carlini and Farid~\cite{carlini2020evading} has shown that with as little as the ability to flip the lowest bit in each pixel, deepfake images can be attacked to evade detection by modern DNN deepfake detection classifiers (e.g., those from Frank et al.~\cite{frank2020leveraging} and Wang et al.~\cite{wang2020cnn}). Neekhara et al.~\cite{neekhara2021adversarial} have also explored black-box attacks and Universal Adversarial Perturbation~\cite{moosavi2017universal} style attacks on deepfake detection. 

% We show that our defense is more robust to adversarial examples than existing frequency-based detection. 

\noindent\textbf{Detecting Adversarial Deepfakes.}
A widely accepted solution to countering adversarial examples is to train the model on adversarial examples, generated during training \citep{madry2018towards}. However,~\citet{carlini2020evading} suggest that adversarial training alone is unlikely to achieve significant improvement in robustness in the difficult deepfake detection setting. Our experiments in Section~\ref{sec:robustness_results} confirm that~\citet{frank2020leveraging}'s frequency-space deepfake detector, even when adversarially trained, cannot withstand deepfake examples crafted using a variety of attacks (see Table~\ref{tab:eval_linf}). While we also adversarially train each model in our ensembles, we find that our ensembles significantly improve robustness over a standalone adversarially trained model (see Section~\ref{sec:robustness_results}).

%\noindent\textbf{Ensemble Defenses.} \label{sec:rel_work_ensemble}

Another class of defenses focuses on removing the effect of the adversarial perturbation without any changes made to the underlying detection technique --- unfortunately, these approaches are computationally intensive, e.g., upto 30 minutes per image~\citep{gandhi2020adversarial, jiang2021residual}, in comparison to %instantaneous time for a forward-pass
no additional overhead in \name. Nevertheless, both approaches are complementary in that pre-processing could be combined with adversarially robust deepfake detectors.
%Initial attempts at defending against adversarial deepfakes have proposed inference-time defenses --- unfortunately, these approaches are computationally intensive, e.g., upto 30 minutes per image~\citep{gandhi2020adversarial, jiang2021residual}.
%Another class of defenses have considered traditional ensembles (of multiple DNNs) --- our discussion towards the end of this section highlights the shortcomings of such standard ensembling, i.e., sharing of non-robust features.    % Our work targets this limitation by improving the adversarial robustness of deepfake detection (see Section~\ref{sec:motivation_design} for detailed methodology). % We propose \name, a framework that leverages the DCT-induced frequency spectrum by intelligently distributing frequency components amongst multiple models to create an ensemble of performant detectors.

Another approach is to use an ensemble of models~\citep{pang2019improving, kariyappa2019improving, yang2021trs} --- in principle, the adversary is then forced to attack multiple models, instead of just one. However,~\citet{he2017adversarial} have shown that arbitrarily ensembling models does not necessarily lead to more robustness. One reason for this (as per ~\citet{ilyas2019adversarial}) is that each model tends to learn the same non-robust features, i.e., an adversary is able to perturb the same features to evade all models. 
% Recent efforts at adversarially robust ensembles have attempted to mitigate this phenomenon by introducing additional regularizers to the training process~\citep{pang2019improving, kariyappa2019improving, yang2021trs}. 
% In contrast, \name bypasses this phenomenon by disjointly partitioning features amongst models, thereby outperforming these approaches (see Section~\ref{sec:robustness_results}).

More recently,~\citet{dutta2021ensembledet} proposed EnsembleDet as defense against adversarial deepfakes. EnsembleDet ensembles different DNN architectures as a defense, and posits that the different architectures will learn different features, providing for improved robustness. We differ from EnsembleDet philosophically, in that we do not require different architectures to avoid learning the same features --- we instead leverage artifact redundancy to design frequency-partitioned ensembles (see Section~\ref{sec:motivation_design} for a more detailed explanation). Furthermore, \name's partitioning approach to achieve disjoint ensembles is novel, and it offers theoretical and empirical advantages where such feature redundancy is available, e.g., GAN-generated deepfakes, allowing it to outperform EnsembleDet (see Section~\ref{sec:robustness_results}). 

\nm{Throw in discussion + cites right here to the few new papers that have popped up. These will be part of our baselines along with EnsembleDet.}


% An alternative to adversarial training is to leverage an ensemble of models --- the adversary is then forced to attack multiple models, instead of just one. However, He et al.~\cite{he2017adversarial} have shown that arbitrarily ensembling models does not necessarily lead to robust defenses --- one reason for this is the {\em transferability shortcoming}, i.e., adversarial examples are often found to transfer between individual models in the ensemble~\cite{wu2020skip}, especially for models with high dimensionality of the adversarial subspace~\cite{tramer2017space}. Recent efforts at adversarially robust ensembles have attempted to mitigate transferability by introducing additional regularizers to the training process~\cite{pang2019improving, kariyappa2019improving, yang2021trs}. In contrast, we achieve zero transferability ``for free" via our frequency-partitioning approach to ensembles (see Section~\ref{sec:motivation_design} for a more detailed explanation).


% By using ensembles over disjoint subsets of features, we avoid transferability between our models, thus increasing robustness.
%To address this, Tramer et al.~\cite{tramer2017ensemble} suggested an ensemble adversarial training method which initially increased robustness to transferred attacks. However, later work by Wu et al.~\cite{wu2020skip} decreased their robustness with improved transfer attacks. 





% In our work, we use adversarial training to train individual models of the ensemble, but we additionally rely on orthogonal gradients to enable the ensemble to be more robust independently of whether or not the models were adversarially trained. In this way, we address the shortcomings of both ensemble defenses and adversarial training by building in disjoint subspaces (such as DCT) into our ensembles to naturally enforce orthogonal gradients.

==> tables/generalization_celeba.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\small
\centering
\begin{tabular}{@{}cccc@{}}
\toprule
\multirow{2}{*}{\textbf{Model}}                 & \multirow{2}{*}{\textbf{Detector}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}No Attack\\ (AP)\end{tabular}}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Attack\\ (ASR)\end{tabular}}} \\
                                                  &                                  & \multicolumn{1}{c}{}                                                                                   &                                                                                     \\ \midrule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{LDM}}} & \textbf{\name (SIZE=1)}                      & 98\%                                                                                              &    95\%                                                                                 \\ 
\multicolumn{1}{c}{}                              & \textbf{\name (SIZE=4)}                 & 93\%                                                                                              &           \textbf{28\%}                                                                          \\ \midrule
\multirow{2}{*}{\textbf{DDIM}}                    & \textbf{\name (SIZE=1)}                      & 98\%                                                                                              &       97\%                                                                              \\ 
                                                  & \textbf{\name (SIZE=4)}                 & 78\%                                                                                              &    \textbf{15\%}                                                                                 \\ \midrule
\multirow{2}{*}{\textbf{PNDM}}                    & \textbf{\name (SIZE=1)}                      &                      97\%                                                                                  &      100\%                                                                               \\  
                                                  & \textbf{\name (SIZE=4)}                 &       97\%                                                                                                 &            \textbf{0\%}                                                                         \\ \bottomrule
\end{tabular}
\caption{\name (SIZE=4) only trained on LSUN Bedroom images is able to generalize its improved robustness to CelebaHQ face images, an entirely different domain unseen during training time.}
\label{tab: generalize_celebahq}
\end{table}

==> tables/natural.tex <==
\begin{table}[]
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccccc}
\toprule
\textbf{Detector}  & \textbf{AT} & \textbf{EnsembleDet} & \textbf{ARDD} & 
\textbf{ARDD-AT} & \textbf{D3-S(4)} \\ \midrule
\textbf{AP} &  98\%   &    100\%       & 100\%    & 100\%     &  93\%       \\ 
\bottomrule
\end{tabular}
}
\caption{Natural performance table : Average Precision}
\end{table}
